Data-Driven Analysis of Pareto Set Topology

When and why can evolutionary multi-objective optimization (EMO) algorithms cover the entire Pareto set? That is a major concern for EMO researchers and practitioners. A recent theoretical study revealed that (roughly speaking) if the Pareto set forms a topological simplex (a curved line, a curved triangle, a curved tetrahedron, etc.), then decomposition-based EMO algorithms can cover the entire Pareto set. Usually, we cannot know the true Pareto set and have to estimate its topology by using the population of EMO algorithms during or after the runtime. This paper presents a data-driven approach to analyze the topology of the Pareto set. We give a theory of how to recognize the topology of the Pareto set from data and implement an algorithm to judge whether the true Pareto set may form a topological simplex or not. Numerical experiments show that the proposed method correctly recognizes the topology of high-dimensional Pareto sets within reasonable population size.

==> Makefile <==
#------------------------------------------------------------------------------
# Project settings
#------------------------------------------------------------------------------

# Project name
PROJNAME := paper

TARGETS := $(PROJNAME).pdf

#------------------------------------------------------------------------------
# Latexmk
#------------------------------------------------------------------------------

# Working directory that stores file dependencies
DEPS_DIR := .deps

# The latexmk command
LATEXMK := latexmk -recorder -use-make -deps \
    -e 'warn qq(In Makefile, turn off custom dependencies\n);' \
    -e '@cus_dep_list = ();' \
    -e 'show_cus_dep();'

#------------------------------------------------------------------------------
# Latexdiff
#------------------------------------------------------------------------------

# latexdiff command
LATEXDIFF := latexdiff-vc --git --force --flatten -e utf8

# ID of the last tagged revision in git repository
GITLASTTAGID := $(shell git rev-list --tags --max-count=1 2>/dev/null)

# Tag name of the last tagged revision in git repository
GITLASTTAG := $(shell git describe --tags $(GITLASTTAGID) 2>/dev/null)

# Name of the head revision in git repository
GITHEAD := HEAD

# Name of the previous revision in git repository
# Use HEAD^ instead of HEAD~ since HEAD~ doesn't work with latexmk
GITPREV := HEAD^

# Git revision to test latexdiff-vc
GITREVISION := $(GITHEAD)

#------------------------------------------------------------------------------
# Chktex
#------------------------------------------------------------------------------

# chktex command
CHKTEX := chktex

#------------------------------------------------------------------------------
# Lacheck
#------------------------------------------------------------------------------

# lacheck command
LACHECK := lacheck

#------------------------------------------------------------------------------
# Make help
#------------------------------------------------------------------------------

# The position at which command descriptions begin
DESCRIPTION_POS := 9

# 1: Show commands in alphabetical order
# 0: Show commands in defined order
ALPHABETICAL := 0

# Don't touch me
ifneq ($(ALPHABETICAL),0)
    SORT := sort |
endif

#------------------------------------------------------------------------------
# Top-level targets
#------------------------------------------------------------------------------
.PHONY: help all clean install paper latexdiff chktex lacheck

help:                                         ##                     Show this help (default target)
	@grep -hE '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) \
		| $(SORT) awk 'BEGIN {FS = ":.*?## "}; \
		{printf "\033[36m%-$(DESCRIPTION_POS)s\033[0m %s\n", $$1, $$2}'

all: paper latexdiff chktex lacheck           ##                     Make paper, latexdiff, chktex, lacheck

paper: $(TARGETS)                             ##                     Generate the PDF paper

latexdiff: $(PROJNAME)-diff$(GITREVISION).pdf ## [GITREVISION=HEAD]  Diff papers in workspace and in git repository

chktex: $(PROJNAME).chktex                    ##                     Check latex syntax by chktex

lacheck: $(PROJNAME).lacheck                  ##                     Check latex syntax by lacheck

clean:                                        ##                     Delete files that are created by running make
	latexmk -C
	$(RM) $(PROJNAME)-diff*.tex *.chktex *.lacheck
	$(RM) -r $(DEPS_DIR)

install:                                      ## [DOCSUFFIX=]        Copy the PDF paper to ../doc/
	mkdir -p ../doc
	cp $(PROJNAME).pdf ../doc/$(PROJNAME)-$(DOCSUFFIX).pdf

archive: paper clean                           ##                     Archive documentation
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip: paper clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

#------------------------------------------------------------------------------
# Sub-level targets
#------------------------------------------------------------------------------

# Dependencies for tex sources
$(foreach file,$(TARGETS),$(eval -include $(DEPS_DIR)/$(file)P))

# PDF papers
%.pdf: %.tex
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	$(LATEXMK) -deps-out=$(DEPS_DIR)/$@P $<

# PDF figures
%.pdf : %.fig
	fig2dev -Lpdf $< $@

# Latexdiff result sources
$(PROJNAME)-diff$(GITREVISION).tex: $(PROJNAME).tex
	$(LATEXDIFF) -r $(GITREVISION) $<

# Checktex log
$(PROJNAME).chktex: $(PROJNAME).tex
	$(CHKTEX) $< | tee $@
	test ! -s $@

# Lacheck log
$(PROJNAME).lacheck: $(PROJNAME).tex
	$(LACHECK) $< | tee $@
	test ! -s $@

# Dependency directory
$(DEPS_DIR):
	mkdir $@

